MAD Max Beyond Single-Node: Enabling Large Machine Learning Model Acceleration on Distributed Systems

Training and deploying large-scale machine learning models is time-consuming, requires significant distributed computing infrastructures, and incurs high operational costs. Our analysis, grounded in real-world large model training on datacenter-scale infrastructures, reveals that 14~32% of all GPU hours are spent on communication with no overlapping computation. To minimize this outstanding communication latency and other inherent at-scale inefficiencies, we introduce an agile performance modeling framework, MAD-Max. This framework is designed to optimize parallelization strategies and facilitate hardware-software co-design opportunities. Through the application of MAD-Max to a suite of real-world large-scale ML models on state-of-the-art GPU clusters, we showcase potential throughput enhancements of up to 2.24x for pre-training and up to 5.2x for inference scenarios, respectively.

==> tables/related_work.tex <==
\begin{table*}[t!]
\begin{center}\resizebox{\linewidth}{!}{
\begin{tabular}{|c||c|c|c|c|c|c|c|}
\hline
\textbf{Prior Work}                                                    & \textbf{Solution Type}                                                                                      & \textbf{Use-Cases}                                                                    & \textbf{\begin{tabular}[c]{@{}c@{}}Evaluated\\ Workloads\end{tabular}}                       & \textbf{\begin{tabular}[c]{@{}c@{}}Parallelization\\ Strategies\end{tabular}}        & \textbf{\begin{tabular}[c]{@{}c@{}}Comms-Compute\\ Overlap\end{tabular}} & \textbf{Hardware}                                                   & \textbf{Validation}                                                                                  \\ \hline\hline
GShard {[}32{]}                                                        & \begin{tabular}[c]{@{}c@{}}XLA compiler\\ extensions\end{tabular}                                           & Training                                                                              & Transformer-MoE                                                                              & \begin{tabular}[c]{@{}c@{}}(operator-level)\\ DP, TP\end{tabular}                    & No                                                                       & TPU                                                                 & \begin{tabular}[c]{@{}c@{}}2K TPU \\ training\end{tabular}                                           \\ \hline
GSPMD {[}68{]}                                                         & \begin{tabular}[c]{@{}c@{}}XLA compiler\\ extensions\end{tabular}                                           & Training                                                                              & \begin{tabular}[c]{@{}c@{}}Transformer,\\ Conformer,\\ Transformer-MoE\end{tabular}          & DP, TP, pipeline                                                                     & No                                                                       & \begin{tabular}[c]{@{}c@{}}TPU\\ (GPU via XLA)\end{tabular}         & \begin{tabular}[c]{@{}c@{}}2K TPU\\ training\end{tabular}                                            \\ \hline
Syndicate {[}34{]}                                                     & Collective scheduling                                                                                       & Training                                                                              & DLRM                                                                                         & \begin{tabular}[c]{@{}c@{}}DP, TP,\\ FSDP, Hybrid\end{tabular}                       & Yes                                                                      & GPU                                                                 & \begin{tabular}[c]{@{}c@{}}128-GPU\\ training\end{tabular}                                           \\ \hline
Themis {[}53{]}                                                        & Collective scheduling                                                                                       & Training                                                                              & \begin{tabular}[c]{@{}c@{}}ResNet, DLRM, \\ Transformer\end{tabular}                         & DP, TP, Hybrid                                                                       & Yes                                                                      & NPU                                                                 &                                                                                                      \\ \hline
Alpa {[}75{]}                                                          & Novel compiler                                                                                              & Training                                                                              & \begin{tabular}[c]{@{}c@{}}ResNet, Transformer,\\ Transformer-MoE\end{tabular}               & \begin{tabular}[c]{@{}c@{}}(operator-level)\\ DP, TP\end{tabular}                    & No                                                                       & GPU                                                                 & \begin{tabular}[c]{@{}c@{}}64-GPU\\ training\end{tabular}                                            \\ \hline\hline
Flexflow {[}24{]}                                                      & \begin{tabular}[c]{@{}c@{}}Simulator, search\\ space explorer\end{tabular}                                  & Training                                                                              & ResNet, RNN, LSTM                                                                            & \begin{tabular}[c]{@{}c@{}}(operator-level)\\ DP, TP\end{tabular}                    & Yes                                                                      & GPU                                                                 & \begin{tabular}[c]{@{}c@{}}64-GPU\\ training\end{tabular}                                            \\ \hline
Pope. et. al {[}49{]}                                                  & \begin{tabular}[c]{@{}c@{}}TPU, Transformer\\ analytical model\end{tabular}                                 & Inference                                                                             & Transformer                                                                                  & \begin{tabular}[c]{@{}c@{}}(operator-level)\\ DP, TP, FSDP\end{tabular}              & Yes                                                                      & TPU                                                                 & \begin{tabular}[c]{@{}c@{}}64-TPU\\ inference\end{tabular}                                           \\ \hline
Pati. et. al. {[}46{]}                                                 & \begin{tabular}[c]{@{}c@{}}Transformer DP,TP\\ analytical model\end{tabular}                                & \begin{tabular}[c]{@{}c@{}}Training,\\ inference\end{tabular}                         & Transformer                                                                                  & DP, TP                                                                               & \begin{tabular}[c]{@{}c@{}}Yes\\ (only DP, TP)\end{tabular}              & GPU                                                                 & \begin{tabular}[c]{@{}c@{}}4-GPU GEMM,\\ AllReduce\end{tabular}                                      \\ \hline
ASTRA-Sim {[}52{]}                                                     & Simulator                                                                                                   & \begin{tabular}[c]{@{}c@{}}Training,\\ inference\end{tabular}                         & ResNet, Transformer                                                                          & \begin{tabular}[c]{@{}c@{}}DP, TP, pipeline,\\ hybrid\end{tabular}                   & Yes                                                                      & NPU                                                                 &                                                                                                      \\ \hline
ASTRA-Sim 2.0 {[}65{]}                                                 & \begin{tabular}[c]{@{}c@{}}Simulator, PyTorch\\ graph interface\end{tabular}                                & \begin{tabular}[c]{@{}c@{}}Training,\\ inference\end{tabular}                         & DLRM, Transformer                                                                            & \begin{tabular}[c]{@{}c@{}}DP, TP, pipeline,\\ hybrid,(operator-level)\end{tabular}  & Yes                                                                      & NPU                                                                 & \begin{tabular}[c]{@{}c@{}}16-GPU\\ AllReduce\end{tabular}                                           \\ \hline
Mystique {[}33{]}                                                      & \begin{tabular}[c]{@{}c@{}}Benchmark creation\\ (from PyTorch traces)\\ for device-level util.\end{tabular} & \begin{tabular}[c]{@{}c@{}}Training,\\ inference\end{tabular}                         & ResNet, DLRM                                                                                 & \begin{tabular}[c]{@{}c@{}}DP (focus on \\ device-level metrics)\end{tabular}        & No                                                                       & GPU                                                                 & \begin{tabular}[c]{@{}c@{}}64-GPU\\ training\end{tabular}                                            \\ \hline
Chakra {[}57{]}                                                        & \begin{tabular}[c]{@{}c@{}}Benchmark creation\\ (from PyTorch traces)\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}Training,\\ inference\end{tabular}                         & DLRM, Transformer                                                                            & \begin{tabular}[c]{@{}c@{}}DP, TP, pipeline,\\ hybrid, (operator-level)\end{tabular} & Yes                                                                      & NPU                                                                 & (see {[}65{]})                                                                                       \\ \hline\hline
\textbf{\begin{tabular}[c]{@{}c@{}}MAD-Max\\ (This Work)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Performance Model,\\ Simulator\end{tabular}}                             & \textbf{\begin{tabular}[c]{@{}c@{}}Training,\\ inference,\\ fine-tuning\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}DLRM-(Transformer, MoE)\\ Transformer-(MoE)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}(layer-type) DP, TP,\\ FSDP, Hybrid\end{tabular}} & \textbf{Yes}                                                             & \textbf{\begin{tabular}[c]{@{}c@{}}NPU,\\ GPU (tuned)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}128, 2K-GPU training \\ (DLRM, LLM) - incl. overlap\end{tabular}} \\ \hline
\end{tabular}}
\end{center}
\caption{Table of select related work. Top block is for parallelization strategy exploration and bottom block is for distributed AI performance modeling.}
\label{tbl:related_work}
\end{table*}

==> tables/related_work_abridged.tex <==
\begin{table*}[t!]
\begin{center}\resizebox{\linewidth}{!}{
\begin{tabular}{|c||cccc|c|c|}
\hline
\multirow{2}{*}{\textbf{Prior Work}}                                   & \multicolumn{4}{c|}{\textbf{Evaluated Large-Scale ML Workloads}}                                                                                                                                                                                                                                           & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Comms-Compute\\ Overlap\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Validation Strategy \\ and Experiments\end{tabular}}} \\ \cline{2-5}
                                                                       & \multicolumn{1}{c|}{\textbf{Transformer}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Transformer-Variants\\ (Conformer, Transformer-MoE)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{DLRM}} & \textbf{\begin{tabular}[c]{@{}c@{}}DLRM-Variants\\ (DLRM-Transformer,\\ DLRM-MoE)\end{tabular}} &                                                                                           &                                                                                                          \\ \hline\hline
GShard {[}32{]}                                                        & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{v}                                                                                                    & \multicolumn{1}{c|}{}              &                                                                                               &                                                                                           & \begin{tabular}[c]{@{}c@{}}2K TPU \\ training\end{tabular}                                               \\ \hline
GSPMD {[}68{]}                                                         & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{v}                                                                                                    & \multicolumn{1}{c|}{}              &                                                                                               &                                                                                           & \begin{tabular}[c]{@{}c@{}}2K TPU\\ training\end{tabular}                                                \\ \hline
Syndicate {[}34{]}                                                     & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{v}             &                                                                                               & v                                                                                         & \begin{tabular}[c]{@{}c@{}}128-GPU\\ training\end{tabular}                                               \\ \hline
Themis {[}53{]}                                                        & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{v}             &                                                                                               & \begin{tabular}[c]{@{}c@{}}v (unvalidated, \\ see {[}52, 65{]})\end{tabular}              & (see {[}65{]})                                                                                           \\ \hline
Alpa {[}75{]}                                                          & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{v}                                                                                                    & \multicolumn{1}{c|}{}              &                                                                                               &                                                                                           & \begin{tabular}[c]{@{}c@{}}64-GPU\\ training\end{tabular}                                                \\ \hline\hline
Flexflow {[}24{]}                                                      & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{}              &                                                                                               & v                                                                                         & \begin{tabular}[c]{@{}c@{}}64-GPU\\ training\end{tabular}                                                \\ \hline
Pope. et. al {[}49{]}                                                  & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{}              &                                                                                               & v (TPU only)                                                                              & \begin{tabular}[c]{@{}c@{}}64-TPU\\ inference\end{tabular}                                               \\ \hline
Pati. et. al. {[}46{]}                                                 & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{}              &                                                                                               & \begin{tabular}[c]{@{}c@{}}v (GPU w/ pure-DP,TP \\ only, unvalidated)\end{tabular}        & \begin{tabular}[c]{@{}c@{}}4-GPU GEMM,\\ AllReduce\end{tabular}                                          \\ \hline
ASTRA-Sim {[}52{]}                                                     & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{v}             &                                                                                               & \begin{tabular}[c]{@{}c@{}}v (unvalidated, \\ see {[}65{]})\end{tabular}                  & (see {[}65{]})                                                                                           \\ \hline
ASTRA-Sim 2.0 {[}65{]}                                                 & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{v}             &                                                                                               & v (unvalidated)                                                                           & \begin{tabular}[c]{@{}c@{}}16-GPU\\ AllReduce\end{tabular}                                               \\ \hline
Mystique {[}33{]}                                                      & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{v}             &                                                                                               &                                                                                           & \begin{tabular}[c]{@{}c@{}}64-GPU\\ training\end{tabular}                                                \\ \hline
Chakra {[}57{]}                                                        & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{v}             &                                                                                               & \begin{tabular}[c]{@{}c@{}}v (unvalidated, \\ see {[}52, 65{]})\end{tabular}              & (see {[}65{]})                                                                                           \\ \hline\hline
\textbf{\begin{tabular}[c]{@{}c@{}}MAD-Max\\ (This Work)\end{tabular}} & \multicolumn{1}{c|}{\textbf{v}}           & \multicolumn{1}{c|}{\textbf{v}}                                                                                           & \multicolumn{1}{c|}{\textbf{v}}    & \textbf{v}                                                                                    & \textbf{v (Figure 7)}                                                                     & \textbf{\begin{tabular}[c]{@{}c@{}}128, 2K-GPU training\\ (DLRM, Transformer,\\ Table 1)\end{tabular}}    \\ \hline
\end{tabular}}
\end{center}
\caption{Select related work. Top block is for parallelization strategy exploration and bottom block is for distributed AI performance modeling.}
\label{tbl:related_work}
\end{table*}

==> tables/related_work_abridged_bottom.tex <==
\begin{table*}[t!]
\begin{center}\resizebox{\linewidth}{!}{
\begin{tabular}{|c||cccc|c|c|}
\hline
\multirow{2}{*}{\textbf{Prior Work}}                                   & \multicolumn{4}{c|}{\textbf{Evaluated Large-Scale ML Workloads}}                                                                                                                                                                                                                                           & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Comms-Compute\\ Overlap\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Validation Strategy \\ and Experiments\end{tabular}}} \\ \cline{2-5}
                                                                       & \multicolumn{1}{c|}{\textbf{Transformer}} & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Transformer-Variants\\ (Conformer, Transformer-MoE)\end{tabular}}} & \multicolumn{1}{c|}{\textbf{DLRM}} & \textbf{\begin{tabular}[c]{@{}c@{}}DLRM-Variants\\ (DLRM-Transformer,\\ DLRM-MoE)\end{tabular}} &                                                                                           &                                                                                                          \\ \hline\hline
Flexflow~\cite{jia2018flexflow}                                                      & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{}              &                                                                                               & v                                                                                         & \begin{tabular}[c]{@{}c@{}}64-GPU\\ training\end{tabular}                                                \\ \hline
Pope. et. al.~\cite{pope2022efficiently}                                                  & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{}              &                                                                                               & v (TPU only)                                                                              & \begin{tabular}[c]{@{}c@{}}64-TPU\\ inference\end{tabular}                                               \\ \hline
Pati. et. al.~\cite{pati2023computation}                                                 & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{}              &                                                                                               & \begin{tabular}[c]{@{}c@{}}v (GPU w/ pure-DP,TP \\ only, unvalidated)\end{tabular}        & \begin{tabular}[c]{@{}c@{}}4-GPU GEMM,\\ AllReduce\end{tabular}                                          \\ \hline
ASTRA-Sim~\cite{rashidi2020astrasim}                                                     & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{v}             &                                                                                               & \begin{tabular}[c]{@{}c@{}}v (unvalidated, \\ see~\cite{won2023astrasim2})\end{tabular}                  & (see~\cite{won2023astrasim2})                                                                                           \\ \hline
ASTRA-Sim 2.0~\cite{won2023astrasim2}                                                 & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{v}             &                                                                                               & v (unvalidated)                                                                           & \begin{tabular}[c]{@{}c@{}}16-GPU\\ AllReduce\end{tabular}                                               \\ \hline
Mystique~\cite{liang2023mystique}                                                      & \multicolumn{1}{c|}{}                     & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{v}             &                                                                                               &                                                                                           & \begin{tabular}[c]{@{}c@{}}64-GPU\\ training\end{tabular}                                                \\ \hline
Chakra~\cite{sridharan2023chakra}                                                        & \multicolumn{1}{c|}{v}                    & \multicolumn{1}{c|}{}                                                                                                     & \multicolumn{1}{c|}{v}             &                                                                                               & \begin{tabular}[c]{@{}c@{}}v (unvalidated, \\ see~\cite{rashidi2020astrasim, won2023astrasim2})\end{tabular}              & (see~\cite{won2023astrasim2})                                                                                           \\ \hline\hline
\textbf{\begin{tabular}[c]{@{}c@{}}MAD-Max\\ (This Work)\end{tabular}} & \multicolumn{1}{c|}{\textbf{v}}           & \multicolumn{1}{c|}{\textbf{v}}                                                                                           & \multicolumn{1}{c|}{\textbf{v}}    & \textbf{v}                                                                                    & \textbf{v (Figure~\ref{fig:dlrma_validation})}                                                                     & \textbf{\begin{tabular}[c]{@{}c@{}}128, 2K-GPU training\\ (DLRM, Transformer,\\ Table~\ref{tbl:method_validation})\end{tabular}}    \\ \hline
\end{tabular}}
\end{center}
\caption{Related work for distributed AI performance modeling.}
\label{tbl:related_work}
\vspace{-5mm}
\end{table*}
